Finite-Time Analysis of Asynchronous Q-learning under Diminishing Step-Size from Control-Theoretic View

Q-learning has long been one of the most popular reinforcement learning algorithms, and theoretical analysis of Q-learning has been an active research topic for decades. Although researches on asymptotic convergence analysis of Q-learning have a long tradition, non-asymptotic convergence has only recently come under active study. The main goal of this paper is to investigate new finite-time analysis of asynchronous Q-learning under Markovian observation models via a control system viewpoint. In particular, we introduce a discrete-time time-varying switching system model of Q-learning with diminishing step-sizes for our analysis, which significantly improves recent development of the switching system analysis with constant step-sizes, and leads to \(\mathcal{O}\left( \sqrt{\frac{\log k}{k}} \right)\) convergence rate that is comparable to or better than most of the state of the art results in the literature. In the mean while, a technique using the similarly transformation is newly applied to avoid the difficulty in the analysis posed by diminishing step-sizes. The proposed analysis brings in additional insights, covers different scenarios, and provides new simplified templates for analysis to deepen our understanding on Q-learning via its unique connection to discrete-time switching systems.

==> experiment/experiment.tex <==

\begin{figure}[h]
     \centering
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Imgs/Q.png}
         \caption{step size = \(\frac{50}{k+100} \)}
         \label{}         
     \end{subfigure}
          \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Imgs/Q_slower.png}
         \caption{step size = \(\frac{200}{k+400}\)}
         \label{}         
     \end{subfigure}
\end{figure}

\begin{figure}[h]
     \centering
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Imgs/results_different_ss.png}
         \caption{Last Iterate}
         \label{}         
     \end{subfigure}
          \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Imgs/rp_results_different_ss.png}
         \caption{Averaged Iterate}
         \label{}         
     \end{subfigure}
\end{figure}

\begin{figure}[h]
     \centering
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Imgs/effective_horizon.png}
         \caption{Effective horizon and eigenvalue of \(G\)}
         \label{}         
     \end{subfigure}
          \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Imgs/gamma_eigenvalues.png}
         \caption{\(\gamma\) and  eigenvalue of \(G\)}
         \label{}         
     \end{subfigure}
\end{figure}


\clearpage


==> introduction/convergence_rate_table.tex <==
\begin{center}
\begin{tabular}{||c c c c||} 
 \hline
 \Cite{even2003learning} & O() & Settings \\ [0.5ex] 
 \hline\hline
 1 & 6 & 87837 & 787 \\ 
 \hline
 2 & 7 & 78 & 5415 \\
 \hline
 3 & 545 & 778 & 7507 \\
 \hline
 4 & 545 & 18744 & 7560 \\
 \hline
 5 & 88 & 788 & 6344 \\ [1ex] 
 \hline
\end{tabular}
\end{center}

==> lower_system/similarity_transform.tex <==
~\cite{lakshminarayanan2018linear} uses similarity transform of Hurwitz matrix to symmetric negative definite matrix. We adopt this technique to bound the \(l2\)-norm of the system matrix which corresponds to the largest singular value.

%%% Discrete Time Version %%%
 
Next we show that the similarity matrix of \(T_{Q^*}\), \(B\) is negative definite.
\begin{lemma}
\(B\) is negative definite matrix.
\end{lemma}

\begin{proof}
If \(B+B^T\) is negative definite, then \(B\) becomes negative definite matrix.
\begin{align*}
    B +B^T = G^{-1/2}( GT_{Q^*}^T +  T_{Q^*} G  )G^{-1/2} = - G^{-1}
\end{align*}
Since \(G^{-1}\) is positive definite matrix, \(B\) becomes negative definite matrix.
\end{proof}


==> markovian/markovian.tex <==
In the previous section, our analysis was based on i.i.d. observation model. However, in real-world scenarios, the state-action tuple follows Markovian observation model. In this section, we assume that the state-action pair follows a Markov chain as summarized in~\Cref{sec:revisit-Q-learning}. The corresponding Q-learning algorithm with Markovian observation model in~\cref{algo:standard-Q-learning2} can be written as follows:
\begin{equation}\label{eq:q_learning_sa}
    Q_{k+1} = Q_k +\alpha_k (D_\infty R + \gamma D_\infty P\Pi_{Q_k}-D_\infty Q_k + w_k(Q_k)) ,
\end{equation}
where $D_\infty  \in {\mathbb R}^{|{\cal S}||{\cal A}| \times |{\cal S}||{\cal A}|}$ is a diagonal matrix with diagonal elements being the stationary state-action distributions, i.e., 
\begin{align*}
(e_s  \times e_a )^{\top} D_\infty  (e_s  \times e_a ) = \mu _\infty  (s,a) = \lim_{k \to \infty } {\mathbb P}[s_k  = s,a_k  = a|\beta ],
\end{align*}
and
\begin{align*}
    w_k(Q_k) &:= (e_{a_k} \otimes e_{s_k} ) (e_{a_k} \otimes e_{s_k})^{\top} R + \gamma (e_{a_k} \otimes e_{s_k})(e_{s_{k+1}})^{\top}\Pi_{Q_k}Q_k\\
    &- (e_{a_k} \otimes e_{s_k})(e_{a_k}\otimes e_{s_k})^{\top} Q_k\\
    &- (D_\infty R+ \gamma D_\infty P\Pi_{Q_k}Q_k - D_\infty Q_k)
\end{align*}
is a noise term. Note that in this section, the notation for the noise term, $w_k(Q_k)$, specifies its dependence on $Q_k$ in order to avoid potential confusions. Using the Bellman equation in~\eqref{eq:bellman_optimal_q}, one can readily prove that the error term \(Q_k - Q^* \) evolves according to the following error dynamic system:
\begin{align*}
 Q_{k+1}-Q^* =    A_{Q_k,k}(Q_k - Q^*)+b_{Q_k,k}+\alpha_k w_k(Q_k),
\end{align*}
where
\begin{align}\label{def:A,b}
    A_{Q,k} &:= I+\alpha_k T_{Q} \quad b_{Q,k}:= \alpha_k  \gamma D_\infty P(\Pi_Q - \Pi_{Q^*})Q^* \\
    T_{Q} &:= \gamma D_\infty P\Pi_{Q}-D_\infty \nonumber.
\end{align}

Note that we can view \(A_{Q,k}\) as a system matrix of a stochastic linear time-varying switching system as in the previous section. Moreover, if the Markov chain does not start from the stationary distribution, the noise term is biased, i.e., \( \mathbb{E}[w_k(Q_k)|\mathcal{F}_k]\neq 0 \), where \(\mathcal{F}_k\) is defined in~\Cref{sec:revisit-Q-learning}. Therefore, the so-called crossing term in~\eqref{eq:v_low_expand}
\begin{align}\label{neq:gradient_bias}
   \xi_k(z_k,Q_k) :=  \xi(z_k,Q_k,o_k) := z^{\top}_kX_k^{\top}G^{1/2}w_k(Q_k).
\end{align} 
is not zero, where \( o_k := (s_k,a_k,r_{k+1},s_{k+1}) \) is the observation, which is the main difference compared to the analysis in the previous section. To resolve the difficulty, in this paper, we assume that the distribution $\mu_k$ mixes in a geometric rate to the stationary distribution \(\mu_\infty\), i.e., $\mu_k \to \mu_\infty$ as $k \to \infty$ exponentially. Note that this assumption is standard and common in the literature~\Cite{sun2018markov,bhandari2018finite,duchi2012ergodic,chen2021lyapunov,li2020sample}, which study stochastic optimization algorithms with Markovian observation models. With the help of geometric mixing rate of the underlying Markov chain, our aim is to bound~\eqref{neq:gradient_bias} by \( \mathcal{O}\left(\frac{\tau^{\mix}(\alpha_k)}{k}\right)\) where \( \tau^{\mix}(\alpha_k)\) is called the mixing-time and will be defined soon later. The previous study in~\Cite{bhandari2018finite} has proved that such biased noise in standard TD-learning can be bounded by \( \mathcal{O}\left(\frac{\tau^{\mix}(\alpha_k)}{k}\right) \) with an additional projection step. In this paper, we prove that with our setups, we can easily follow the spirits of~\Cite{bhandari2018finite}, and prove convergence of Q-learning without the additional projection step.


Finally, in this section, we separate the index of the observation \(\{o_k\}_{k=1}^{n}\)and the iterate \( \{Q_k \}_{k=1}^{n} \) in the noise term, i.e.,
\begin{align*}
    w_j(Q_i) &:= (e_{a_j} \otimes e_{s_j} ) (e_{a_j} \otimes e_{s_j})^{\top} R + \gamma (e_{a_j} \otimes e_{s_j})(e_{s_{j+1}})^{\top}\Pi_{Q_i}Q_i\\
    &- (e_{a_j} \otimes e_{s_j})(e_{a_j}\otimes e_{s_j})^{\top} Q_i \\
    &- (D_\infty R+ \gamma D_\infty P\Pi_{Q_i}Q_i - D_\infty Q_i).
\end{align*}
Moreover, we will use the notation \(w(o_j,Q_i):=w_j(Q_i)\) interchangeably in order to specify the dependence of the noise on the observation. The subscript of \(w_j\) indicates the time index of observation, while the subscript of $Q_i$ is the time index corresponding to Q-iteration. When their indices coincide, that is, having both  \(k\)-th observation of \(\{o_k\}_{k=1}^{n}\) and \(k\)-the iterate of \( \{Q_k \}_{k=1}^{n} \), we use \(w_k\). Before we proceed on, let us summarize some information theoretic results from~\Cite{bhandari2018finite} in the following subsection.


\subsection{Preliminaries on information theoretic results}\hfill\\

In this section, we introduce some definitions used in information theory, and its relation to the Markov chain under our consideration.
\begin{definition}[Total variation distance~\Cite{levin2017markov}]
The total variation distance between two probability distributions \(P\) and \(Q\) on the sample space, \(\Omega\), is defined as
\begin{align*}
    d_{TV}(P,Q) := \max_{A\in \Omega} | P(A) - Q(A)|.
\end{align*}
\end{definition}

\begin{definition}[Conditional independence~\Cite{koller2009probabilistic}]\label{def:conditional-independence}
For random variables X,Y, and Z, 
\begin{align*}
    X \to Y \to Z
\end{align*}
denotes that \(X\) and \(Z\) are conditionally independent given \(Y\), that is, ${\mathbb P}(Z|X,Y) = {\mathbb P}(Z|Y)$.
\end{definition}
%Now, let us assume standard assumptions on Markov chain throughout the analysis.

With~\Cref{assmp:irreducible_aperiodic}, the Markov chain reaches its stationary distribution at a geometric rate. We note that most of the analysis of stochastic optimization on Markov chain~\Cite{sun2018markov,bhandari2018finite,duchi2012ergodic} relies on geometric convergence to the stationary distribution. Our analysis also adopts this standard scenario. 
%We believe our analysis can be also extended to non-ergodic sense~\Cite{sun2018markov}.
\begin{lemma}[\Cite{levin2017markov}]\label{assumption:mixing}
Under~\Cref{assmp:irreducible_aperiodic}, there exist constants \(m>0\) and \( \rho \in (0,1) \) such that 
% \begin{equation*}
%     \sup_{(s,a)\in\mathcal{S}\times \mathcal{A}} d_{TV}(\mu_k(s,a),\mu_\infty) \leq m \rho^k, \quad \forall{k} \in \mathbb{N},
% \end{equation*}
\begin{equation*}
     d_{TV}(\mu_k,\mu_\infty) \leq m \rho^k, \quad \forall{k} \in \mathbb{N},
\end{equation*}
where $\mu_k$ and $\mu_\infty$ are defined in~\eqref{eq:mu_k_infty}.
%In addition, the initial distribution of \((s_0,a_0)\) is the steady-state distribution \(\mu\), so \( \{ (s_k,a_k) \}_{k=0}^{\infty} \) is a stationary sequence.
\end{lemma}

Now, we can define the mixing-time as follows:
\begin{align}\label{def:mixing_time}
    \tau^{\mix}(c) := \min \{k\in \mathbb{N} \mid m \rho^k \leq c\},
\end{align}
which is the minimum time required for the total variation distance between the stationary distribution and the current distribution to be less than a desired level $c >0$. Moreover, \(m\) and \(\rho\) are the constants defined in~\Cref{assumption:mixing}.

% Noting that 
% \begin{align}
%  \tau(\alpha) \geq \frac{1}{\log \rho} \log \alpha   + \frac{1}{\log \rho} \log m , \nonumber
% \end{align},
% \(\) can be expressed as 
% \begin{align}
%     \tau(\alpha) = \ceil{\frac{1}{\log \rho} \log \frac{m}{\alpha}} \nonumber.
% \end{align}
Related to the mixing-time, let us introduce the following quantity:
\begin{align}
    K_{\mix} := \min \{ k \mid  t \geq 2 \tau^{\mix}(\alpha_t) , \quad \forall{t\geq k}\} \label{def:K},
\end{align}
{\color{blue}Please keep the consistency: replace $:$ with $|$ and fit the size with the bracket size. }
where \(\alpha_t\) is the step-size defined in~\eqref{eq:step_size}. Note that \( K_{\mix}\) is well-defined, since upper bound of \( \tau^{\mix} (\alpha_k)\) is logarithmically proportional to \(k\). Intuitively, \( K_{\mix}\) roughly means the number of iterations, after which the mixing-time corresponding to the current step-size can be upper bounded by the current time. Therefore, the analysis can be divided into two phases, the first phase $k \le K_{\mix}$ and the second phase $k \ge K_{\mix}$. Note that this approach is common in the literature. For example, the recent paper~\Cite{chen2021lyapunov} derived a convergence rate after \(K_{\mix}\) iterations, and~\Cite{li2020sample} derived a sample complexity after some time related to the mixing time. For \(k \leq K_{\mix}\) , we can ensure the iterate remains bounded, and after \( k \geq K_{\mix}\), we have \(\mathcal{O}\left(\sqrt{\frac{\log k}{k}}\right) \) convergence rate. Lastly, we state a key lemma to prove a bound on~\eqref{neq:gradient_bias} with \(\mathcal{O}\left(\frac{\tau^{\mix}(\alpha_k)}{k}\right) \).
\begin{lemma}[Control of coupling~\Cite{bhandari2018finite}]\label{lem:control_coupling}
For some \( k\geq 0\), and \(\tau > 0 \), consider two random variables \(X\) and \(Y\) such that
\begin{equation*}
    X \to (s_k,a_k) \to (s_{k+\tau},a_{k+\tau}) \to Y.
\end{equation*}
Let the underlying Markov chain, $\{ (s_k ,a_k )\} _{k = 0}^\infty$, satisfies~\Cref{assmp:irreducible_aperiodic}. Moreover, let us construct independent random variables $X'$ and $Y'$ drawn from the
marginal distributions of $X$ and $Y$, respectively, i.e., $X' \sim P(X =  \cdot )$ and $Y' \sim P(Y =  \cdot )$ so that 
\begin{align*}
P(X'=\cdot,Y'=\cdot ) = P(X'=\cdot)P(Y'=\cdot) = P(X=\cdot)  P(Y=\cdot). 
\end{align*}
Then, for any function \(f:\mathcal{X}\times \mathcal{Y}\to\mathbb{R}\) such that \(\sup_{(x,y)\in\mathcal{X} \times \mathcal{Y}} |f(x,y)| < \infty \), we have
\begin{equation*}
    | \mathbb{E} [f(X,Y)] - \mathbb{E}[f(X',Y')]| \leq 2 \sup_{(x,y)\in\mathcal{X}\times \mathcal{Y}} |f(x,y)| (m\rho^{\tau}).
\end{equation*}
\end{lemma}

\begin{proof}
Let \(f_{\infty}:= \sup_{(x,y)\in\mathcal{X}\times \mathcal{Y}} |f(x,y)| \) and \( f^{\prime}(X,Y) = f(X,Y)/f_{\infty} \)
\begin{align}
   | \mathbb{E}[f^{\prime}(X,Y)] -\mathbb{E}[f^{\prime}(X',Y')] | &= \int f dP - \int f dQ \\
   &\leq d_{TV} (P,Q)
   &= I_{TV}(P,Q)
\end{align}
\end{proof}

{\color{teal}The above lemma states that for some functional of sample from Markov chain and its lagged sample, it differs from the functional of independent samples from its stationary distribution by geometric rate.}
% For bounded dynamics, we can bound the difference of expectation with geometric term, which will be shown in the next subsection. 
\subsection{Bounding the crossing term \( \mathbb{E}[\xi_k(z_k,Q_k)] \)}\hfill\\
With our assumptions in place, we are now ready to bound the crossing term, \(\mathbb{E}[\xi_k(z_k,Q_k)]\), provided that the iterate \(z_k\) is bounded. The recent paper~\Cite{bhandari2018finite} uses an additional projection step to keep the iterate bounded for analysis of TD-learning. However, since \(Q^L_k -Q^*\) is always bounded, we can ensure that \(z_k\) is bounded as well without the projection. 
% To see the dependence on \( d_{\min}\) and \(\frac{1}{1-\gamma}\), we assume the following bound throughout the paper:
%  \begin{equation*}
%      ||Q^L_0 -Q^*||_{\infty} \leq \frac{4}{(1-\gamma)^2 d_{\min}} .
%  \end{equation*}
In this section, we need to establish the boundedness of \(Q^L_k - Q^* \). As in~\Cref{assm:Q_0_reward_bound}, we assume that \(||Q^L_0||_{\infty} \leq 1 \). Note that it is always possible because \(||Q_0||_{\infty} \leq 1 \), and we can always set $Q_0 = Q^L_0$ without loss of generality. 
% For \( \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}\), we have the following bound:
% \begin{align}
%      \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} &\leq(|\mathcal{S}||\mathcal{A}|)^{\frac{3}{2}}  (1+ \alpha_0 ||B||
%     _{2})Q^L_{\max}||G||_2 \frac{4}{1-\gamma} \nonumber \\
%     &\leq (|\mathcal{S}||\mathcal{A}|)^{\frac{3}{2}}  (1+ \frac{\theta}{\xi} ||B||_2)\frac{4}{d_{\min}(1-\gamma)^2} \frac{|\mathcal{S}||\mathcal{A}|}{2(1-\gamma)d_{\min}}\frac{4}{1-\gamma} \nonumber\\
%     &\leq  (1+ \frac{\nu}{2\sigma^2(B)_{\max}(|\mathcal{S}||\mathcal{A}|)^2} ||B||_2)
%     \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}
%     \nonumber\\
%     &\leq (1+ \frac{\nu}{2||B||_2(|\mathcal{S}||\mathcal{A}|)^2})
%     \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}
%     \nonumber\\
%     &\leq  (1+ \frac{\nu}{2} \frac{1}{(1-\gamma)d_{\min}|\mathcal{S}||\mathcal{A}|})
%     \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}
%     \nonumber\\
%     &\leq  (1+ \frac{1}{2|\mathcal{S}||\mathcal{A}|})
%     \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}
%     \nonumber\\
%     &\leq  \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}\nonumber
% \end{align}

\begin{lemma}[Boundedness of \(Q^L_k-Q^*\) and \(z_k\)]\label{lem:bound_z_k}
Suppose that \(||Q^L_0||_{\infty} \leq 1 \) holds. Then, the following statements hold true:
 \begin{enumerate}[1)]
     \item  For all \(k\geq 0 \), we have
\begin{align*}
    ||Q_k^L-Q^*||_{\infty} \leq \frac{4}{(1-\gamma)^2 d_{\min}} .
\end{align*}
     \item From item 1), for all \(k\geq 0 \) we have,   
     \begin{align}
    ||z_k||_{\infty} \leq \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{1}{2}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}} \nonumber.
\end{align}
 \end{enumerate}
\end{lemma}

\begin{proof}
We first prove the boundedness of \(Q^k_L-Q^*\) by an induction argument. 
For \(k=0\), we have
 \begin{equation*}
     ||Q^L_0 -Q^*||_{\infty} \leq \frac{4}{(1-\gamma)^2 d_{\min}} .
 \end{equation*}
because
 \begin{align*}
     ||Q^L_0 - Q^*||_{\infty} &\leq ||Q^L_0 ||_{\infty} + ||Q^*||_{\infty}\\
     &\leq 1 + \frac{1}{1-\gamma} \\
     &= \frac{2-\gamma}{1-\gamma} \leq \frac{4}{(1-\gamma)^2 d_{\min}}
 \end{align*}   
 where the last inequality follows from~\Cref{lem:q_k_bound}. Next, suppose that \(||Q^L_k - Q^*||_{\infty} \leq \frac{4}{(1-\gamma)^2 d_{\min}} \) holds for some \(k\geq 0\). Then, we have
\begin{align}
    ||Q^L_{k+1}-Q^*||_{\infty} &\leq ||A_{Q^*,k}||_{\infty} ||Q^L_k -Q^*||_{\infty} +\alpha_k ||w_k||_{\infty} \nonumber \\
                           &\leq (1-d_{\min}(1-\gamma) \alpha_k) ||Q^L_k -Q^*||_{\infty} +\alpha_k \frac{4}{1-\gamma}  \nonumber \\
                           &\leq \frac{4}{d_{\min}(1-\gamma)^2} \nonumber,
\end{align} 
where the first inequality follows from the update of lower comparison system~\eqref{eq:lower_comparison_update}, and the second inequality comes from the bound on \(w_k\) in~\eqref{ineq:bound on w_k} and \(A_{Q^*,k}\) in~\Cref{lem:spectral radius of A}.
Then, the proof is completed by induction. Next, the boundedness of \(z_k\) naturally follows from the coordinate transform in~\eqref{eq:coordinate_transform_sa}. In particular, it follows from the inequalities
\begin{align}
        ||z_k||_{\infty} &\leq ||G^{1/2}||_{\infty} ||Q^L_k-Q^*||_{\infty}\leq  \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{1}{2}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}} \nonumber,
\end{align}
where the second inequality follows from~\Cref{assm:Q_0_reward_bound} and~\Cref{lem:G_upper_bound} to bound $||G^{1/2}||_{\infty}$. This completes the proof.
\end{proof} 

Using the boundedness of \(z_k\) in~\Cref{lem:bound_z_k}, we establish boundedness and Lipschitzness of \(\xi_k\) in the next lemma.
\begin{lemma}[Bound on \(\xi_k\) and Lipschitzness]\label{lem:bdd_xi}\label{lem:lipschitz-xi}\label{lem:lipschitz-xi}
\begin{enumerate}[1)]
    \item The crossing term \(\xi_k(z_k,Q_k)\) at \(k\)-th iterate is always bounded as follows:
   \begin{align}
       |\xi_k(z_k,Q_k)| \leq \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}\nonumber.
   \end{align}
   \item  For any \(k \geq 0\), \(\xi_k(z,Q) \) is Lipschitz with respect to \( (z,Q) \), i.e.,
\begin{align*}
     |\xi_k (z,Q_k) - \xi_k (z',Q')| \leq \frac{16(|\mathcal{S}||\mathcal{A}|)^3}{(1-\gamma)^3d_{\min}^2} ||Q-Q'||_{\infty} + \frac{3|\mathcal{S}||\mathcal{A}|}{2(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{1}{2}}}||z-z'||_{\infty} \nonumber
\end{align*}
\end{enumerate}
\end{lemma}


% \begin{lemma}[Non-randomness of \(z_0\)]\label{lem:non-randomness:z_0}
% For \(k \geq 0 \), we have
% \begin{align}
%     \mathbb{E}[\xi(z_0,\mathcal{O}_k)] = 0. \nonumber
% \end{align}
% \end{lemma}
% \begin{proof}
% Considering non-randomness of \(z_0\), we have
% \begin{align}
%     \mathbb{E}[\xi(z_0,\mathcal{O}_k)] = 0. \nonumber
% \end{align}

% \end{proof}
\begin{lemma}
For \( 0 \leq \tau \leq k \), we have:
\begin{align*}
\mathbb{E}[\xi_k(z_{k},Q_{k})]  &\leq  \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} (m\rho^{k}) \nonumber .
\end{align*}
\end{lemma}
\begin{proof}
Using tower property of expectation, and convexity of \(|\cdot|\), we have the following:
\begin{align}
   | \mathbb{E}[\xi_k(z_{k},Q_{k})]| &=  |\mathbb{E}[\mathbb{E}[\xi_k(z_{k},Q_{k}) |z_{k},Q_{k}]]| \nonumber \\
   &\leq \mathbb{E} [|\mathbb{E}[\xi_k(z_{k},Q_{k}) ||z_{k},Q_{k} ]| ] 
\end{align}
Hence, now our aim is to bound \(|\mathbb{E}[\xi_k(z_{k-\tau},Q_{k-\tau}) ||z_{k-\tau},Q_{k-\tau} ]| \). 
\begin{align*}
    |\mathbb{E}[\xi (z_{k},Q_{k},o_k)|z_{k},Q_{k}]| &=  |\mathbb{E}[(z_{k})^{\top} X^{\top}_k G^{1/2} w(Q_{k},o_k)|z_{k},Q_{k}]| \\
    &= | z^{\top}_{k} X^{\top}_{k}G^{1/2}\mathbb{E}[w(Q_{k},o_k)|z_{k},Q_{k}]|\\
    &=|\mathcal{S}||\mathcal{A}| ||X_k z_{k}||_2 ||G^{1/2}||_2 ||\mathbb{E}[w(Q_{k},o_k) | 
    Q_{k-\tau}]||_{\infty} \\
    &\leq  \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}} \frac{(|\mathcal{S}||\mathcal{A}|)^{\frac{1}{2}}}{(1-\gamma)^{\frac{1}{2}}d_{\min}^{\frac{1}{2}}} \frac{2}{1-\gamma}  m \rho^{k} \\
    &\leq \frac{16(|\mathcal{S}||\mathcal{A}|)^3}{(1-\gamma)^4 d_{\min}^2} m \rho^k
\end{align*}
We first define \(D_{\mu_k}\) to denote the state-action distribution at \(k\)-th time step as follows:
\begin{align*}
(e_s  \times e_a )^{\top} D_{\mu_k}  (e_s  \times e_a ) = \mu _k  (s,a) = {\mathbb P}[s_k  = s,a_k  = a|\beta ]
\end{align*}
\begin{align*}
 ||\mathbb{E}[w(Q_{k},o_k) | Q_{k}]||_{\infty} &= ||(D_{\mu_k}-D_{\infty})(R+\gamma P\Pi_{Q_{k}}Q_{k}-Q_{k}) ||_{\infty} \\
 &\leq ||D_{\mu_k}-D_{\infty}||_{\infty} ||R+\gamma P\Pi_{Q_{k}}Q_{k}-Q_{k}||_{\infty} \\
 &\leq \left(1+\frac{\gamma}{1-\gamma} +\frac{1}{1-\gamma}\right) \sup_{(s,a)\in \mathcal{S}\times \mathcal{A
 }} |\mu_k(s,a)-\mu_{\infty}(s,a) | \\
  &= \left(1+\frac{\gamma}{1-\gamma} +\frac{1}{1-\gamma}\right) d_{TV}(\mu_k,\mu_{\infty}) \\
 &\leq \frac{2}{1-\gamma}m \rho^{k}
\end{align*}
\end{proof}

The proof is given in~\Cref{app:lem:bdd_xi}. Using above results, we are now in position to provide a bound on the crossing term, \(\mathbb{E}[\xi_k(z_{k-\tau},Q_{k-\tau})]\).
\begin{lemma}[Boundedness of {$\mathbb{E}[\xi_k(z_{k-\tau},Q_{k-\tau})]$} ]\label{lem:boundedness_of_ex_xi_k_tau}
For any \(\tau\) and \(k\) such that \( 0 \leq \tau \leq k\), there exist \(m>0\) anr \(0<\rho<1\) such that
\begin{align*}
\mathbb{E}[\xi_k(z_{k-\tau},Q_{k-\tau})]  &\leq  \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} (m\rho^{\tau}) \nonumber .
\end{align*}
\end{lemma}
\begin{proof}
Throughout the proof,~\Cref{lem:control_coupling} will play an important role. To apply~\Cref{lem:control_coupling}, first note the relations
\begin{align}
 (z_{k-\tau},Q_{k-\tau}) \to (s_{k-\tau},a_{k-\tau}) \to (s_k,a_k) \to o_k, \nonumber
\end{align}
where the arrow notation is defined in~\Cref{def:conditional-independence}, and $o_k:= (s_k,a_k, r_{k+1}, s_{k+1})$. Now, let us construct the coupling distribution of \((z_{k-\tau}',Q_{k-\tau}')\) and \(o'_k\) drawn independently from some marginal distributions of \((z_{k-\tau},Q_{k-\tau})\) and \(o_k\), respectively, i.e., $(z_{k - \tau}^{\prime}   ,Q_{k - \tau  }^\prime ) \sim {\mathbb P}((z_{k - \tau } ,Q_{k - \tau } ) =  \cdot )$ and $o_k ' \sim {\mathbb P}(o_k  =  \cdot )$. Then,~\Cref{lem:control_coupling} leads to 
\begin{align}
|{\mathbb E}[\xi (z_{k-\tau} ,Q_{k-\tau},o_k )] - {\mathbb E}[\xi  (z_{k-\tau}',Q'_{k-\tau},o_k ')]| \leq  \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}  m\rho ^\tau  \label{eq:1}
\end{align}
Using tower property of the expectation, \(\mathbb{E}[X]  =\mathbb{E}[\mathbb{E}[X|Y]] \), we have
%Since \((z_{k-\tau}',Q_{k-\tau}')\) and \(o'_k\) are independent, we have 
\begin{align*}
    \mathbb{E}[\xi (z_{k-\tau}',Q_{k-\tau} ',o'_k)] &= \mathbb{E}[{\mathbb E}[(z_{k - \tau } ')^{\top} X_k^{\top} G^{1/2} w(Q'_{k-\tau},o'_k)|z_{k-\tau}',Q_{k-\tau}']]\\
    &= \mathbb E[(z_{k - \tau } ')^{\top} X_k^{\top} G^{1/2} \mathbb{E}[ w(Q'_{k-\tau},o'_k)|z_{k-\tau}',Q_{k-\tau}']] \\
    &\leq || X_k  z^{\prime}||_2 ||G^{1/2}||_2 || |\mathcal{S}||\mathcal{A}| ||\mathbb{E}[w(Q^{\prime}_{k-\tau},o^{\prime}_k')]||_{\infty} \\
    &\leq \frac{8(|\mathcal{S}||\mathcal{A}|)^2}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}}
\end{align*}

{\color{teal}The coupling construction that \((z_{k-\tau}^{\prime},Q_{k-\tau}^{\prime} )\) and \(o_k^{\prime}\) are independent, implies independence of \( Q'_{k-\tau}\) and \(o'_k\). Hence, we have \(\mathbb{E}[w(Q'_{k-\tau},o'_k)|z'_{k-\tau},Q'_{k-\tau}] = 0\).}
%Moreover, if we consider a marginal distribution of \(o_k':= (s_k',a_k', r_{k+1}', s_{k+1}')\) assuming $(s_k',a_k')\sim \mu_{\infty}$ 
\begin{align}
    \mathbb{E} [w(Q^{\prime}_k,o^{\prime}_k)] - \mathbb{E} [w(Q^{\prime}_k,o^{\prime \prime }_k)] & \leq m \rho^k 
\end{align}

{\color{blue} [Please check if we can simply assume $(s_k',a_k')\sim \mu_{\infty}$. In reality, $(s_k',a_k')\sim \mu_k$. If it is an error, 
we can use the fact that $\|\mu_{\infty} - \mu_k\|_\infty$ also converge exponentially]}
%, then ${\mathbb E}[w(Q'_{k-\tau},o'_k)|z_{k-\tau}',Q_{k-\tau}'] = 0$. 
Therefore, 
\begin{align*}
{\mathbb E}[\xi(z_{k-\tau}',Q_{k-\tau}',o_k ')|z_{k-\tau}',Q_{k-\tau}'] = 0. 
\end{align*}
Combining this with~\eqref{eq:1}, we have 
\[
|{\mathbb E}[\xi _k (z_{k - \tau } ,Q_{k-\tau} )]| = |{\mathbb E}[\xi (z_{k - \tau } ,Q_{k-\tau},o_k )] - {\mathbb E}[\xi (z_{k - \tau } ',Q_{k-\tau}',o_k ')]| \le \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} m\rho ^\tau  
\]
which completes the proof. 

The above lemma states that if \(\tau\), the time difference between the new observation \(o_k\) and previous iterate \(Q_{k-\tau}\), is large, then the Markovian noise term \(w(o_k,Q_{k-\tau})\) inherits the geometric mixing property of the Markov chain. Now, combining the above result with Lipschitzness of \(\xi_k (z_k,Q_k)\), we can bound  \(\mathbb{E}[\xi_k(z_k,Q_k)] \) as follows:

%{\color{orange}From the construction, \(z'_{k-\tau}\) and \(\mathcal{O}'_k\) are independent, and when \(z'_{k-\tau}\) is non-random, we %have \(\mathbb{E}[\xi(z'_{k-\tau},\mathcal{O}_k')]=0\). Hence the following equality satisfies:
%\begin{align}
%    \mathbb{E}[\xi(z'_{k-\tau},\mathcal{O}'_k)] 
%    = \mathbb{E}[ \mathbb{E}[\xi(z'_{k-\tau},\mathcal{O}'_k)| z'_{k-\tau} ]] = 0 \nonumber
%\end{align}

%Combining~\Cref{lem:bdd_xi} and~\Cref{lem:control_coupling}, we have
%\begin{align}
%\mathbb{E}[\xi(z_{k-\tau},\mathcal{O}_k)-\xi(z_{k-\tau}',\mathcal{O}_k')] &=\mathbb{E}[\xi(z_{k-\tau},\mathcal{O}_k)]  \nonumber \\
%    &\leq 2  \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} (m\rho^{\tau}) \nonumber .
%\end{align}


\end{proof}


\begin{lemma}[Boundedness of {$\mathbb{E}[\xi_k (z_k,Q_k)]$} ]\label{lem:boundedness_of_ex_z}
% For any \(0 \leq k \leq K\) where \(k\in \mathbb{Z}_+\),and \(K \in \mathbb{Z}_+\),
% \begin{align}
% \mathbb{E}[\xi_k(z_k)] \leq  (2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \alpha_{k^*} \nonumber
% \end{align}
% where \(k^*= \max (0,k-\tau^{\mix}(\alpha_K))\). In addition,
% \begin{align}
%     \mathbb{E}[\xi_k(z_k)] \leq M \sum^{k-1}_{i=0} \alpha_i \nonumber
% \end{align}
% \begin{enumerate}[{1)}]
% \item For \(k \leq K_{\mix}\), we have
% \begin{align}
%      \mathbb{E}[\xi_k (z_k)] &\leq    \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}   K_{\mix}  \alpha_0  \nonumber.
% \end{align}

% \item For \( k \geq K_{\mix}\), we have
% \begin{align}
%     \mathbb{E}[\xi_k (z_k)] &\leq \left( \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} +  \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2} \tau^{\mix}(\alpha_k)\right)\alpha_{k-\tau^{\mix}(\alpha_k)} . \nonumber
% \end{align}
% \end{enumerate}

For \( k \geq K_{\mix}\), expectation of the cross term can be bounded as follows:
\begin{align}
    \mathbb{E}[\xi_k (z_k,Q_k)] &\leq \left( \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} +  \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2} \tau^{\mix}(\alpha_k)\right)\alpha_{k-\tau^{\mix}(\alpha_k)} . \nonumber
\end{align}

\end{lemma}
\begin{proof}
From the update of \(z_i\) in~\eqref{eq:coordinate_transform_sa}, for \(i\geq 0\), we have
\begin{align}
    ||z_{i+1} - z_i ||_{\infty} &= || \alpha_i B z_i + \alpha_i G^{1/2}w_i||_{\infty} \nonumber \\
    &\leq (||B||_{\infty} ||z_i||_{\infty} + ||G^{1/2}||_{\infty }||w_i||_{\infty})\alpha_i \nonumber \\
    &\leq  \left( ||B||_{2}||z_i||_{\infty} + ||G^{1/2}||_{2}  \frac{4}{1-\gamma} \right)\alpha_i  \nonumber \\
    &\leq \left((1-\gamma)d_{\min}(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{4}} \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{1}{2}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}} + \sqrt{\frac{|\mathcal{S}||\mathcal{A}|}{2(1-\gamma)d_{\min}}} \frac{4}{1-\gamma}\right)\alpha_i \nonumber\\
    &\leq  \frac{16(|\mathcal{S}||\mathcal{A}|)^{\frac{7}{4}}}{(1-\gamma)^{\frac{3}{2}}d_{\min}^{\frac{1}{2}}}\alpha_i  \label{ineq:z-z},
\end{align}
where the second inequality follows from bounding \(w_i\) in~\Cref{lem:w_k_bound}, and the third inequality is obtained by bounding each terms with~\Cref{lem:B_upper_bound} and~\Cref{lem:bound_z_k}. 
Similarly for \(Q_k\), we have
\begin{align}
    ||Q_{i+1}-Q_i||_{\infty} &= \alpha_i||(e_{a_k} \otimes e_{s_k} ) (e_{a_k} \otimes e_{s_k})^{\top} R + \gamma (e_{a_k} \otimes e_{s_k})(e_{s_{k+1}})^{\top}\Pi_{Q_k}Q_k \nonumber\\
    &- (e_{a_k} \otimes e_{s_k})(e_{a_k}\otimes e_{s_k})^{\top} Q_k||_{\infty}  \nonumber\\
    &\leq\left(1 + \frac{1}{1-\gamma}\right) \alpha_i . \label{ineq:Q-Q^*}
\end{align}
For any \(k\geq 1\) and \(\tau \) such that  \( 1 \leq \tau \leq k\), summing up~\eqref{ineq:z-z} and~\eqref{ineq:Q-Q^*} from \(i=k -\tau\) to \(k-1\), respectively, we get
\begin{align}
    ||z_k - z_{k-\tau}||_{\infty} &\leq \sum^{k-1}_{i=k-\tau} || z_{i+1}- z_i||_{\infty} \leq \frac{(|\mathcal{S}||\mathcal{A}|)^{\frac{7}{4}}}{(1-\gamma)^{\frac{3}{2}}d_{\min}^{\frac{1}{2}}}  \sum^{k-1}_{i=k-\tau} \alpha_i 
    \label{ineq:z_k_minus_z_k_tau}
\end{align}
and 
\begin{align}
    ||Q_k - Q_{k-\tau}||_{\infty} &\leq \sum^{k-1}_{i=k-\tau} || Q_{i+1}- Q_i||_{\infty} \leq \frac{2-\gamma}{1-\gamma}  \sum^{k-1}_{i=k-\tau} \alpha_i 
    \label{ineq:q_k_minus_q_k_tau}
\end{align}
respectively. Therefore, combining~\Cref{lem:lipschitz-xi},~\eqref{ineq:z_k_minus_z_k_tau}, and~\eqref{ineq:q_k_minus_q_k_tau} lead to
    \begin{align}\label{ineq:xi_1}
        \xi_k (z_k,Q_k) -  \xi_k (z_{k-\tau},Q_{k-\tau}) &\leq \frac{16(|\mathcal{S}||\mathcal{A}|)^3}{(1-\gamma)^3d_{\min}^2}||Q_k-Q_{k-\tau}||_{\infty} \nonumber\\
        &+  \frac{3|\mathcal{S}||\mathcal{A}|}{2(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{1}{2}}}||z_k-z_{k-\tau}||_{\infty} \nonumber\\
        &\leq \frac{32(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}\sum^{k-1}_{i=k-\tau} \alpha_i 
        + \frac{3(|\mathcal{S}||\mathcal{A}|)^{3}}{2(1-\gamma)^4d_{\min}} \sum^{k-1}_{i=k-\tau} \alpha_i \nonumber\\
        &\leq  \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2} \tau \alpha_{k-\tau},
    \end{align}
where the last inequality is due to the fact that \(\alpha_i\) is a non-increasing sequence. Next, we will bound \( \mathbb{E}[\xi_k (z_k,Q_k)]\). In particular, taking total expectations on~\eqref{ineq:xi_1} yields
\begin{align}
       \mathbb{E}[ \xi_k (z_k,Q_k)] \leq \mathbb{E}[\xi_k (z_{k-\tau},Q_{k-\tau})] +   \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}  \tau \alpha_{k-\tau} \nonumber.
\end{align}

% Let \( \tau := \tau^{\mix}(\alpha_k)\), and applying~\Cref{lem:boundedness_of_ex_xi_k_tau}.

% #### bhandari ####

% For \(k \leq \tau^{\mix}(\alpha_K)\), letting \(\tau=k\) , we have
% %\(m\rho^{\tau}< \alpha_K\), we have
% \begin{align}
%     \mathbb{E}[\xi_k (z_k)] &\leq \mathbb{E}[\xi_k (z_{0})] 
%     + \frac{4|\mathcal{S}|^2|\mathcal{A}|^2}{1-\gamma}(1+\alpha_k ||B^{\top}||_{\infty})( ||B||_{\infty}||G^{1/2}||_{\infty}^2 Q^L_{\max} + ||G^{1/2}||_{\infty}^2W )) \tau^{\mix}(\alpha_K) \alpha_0 \nonumber\\
%     &= \frac{4|\mathcal{S}|^2|\mathcal{A}|^2}{1-\gamma}(1+\alpha_k ||B^{\top}||_{\infty})( ||B||_{\infty}||G^{1/2}||_{\infty}^2 Q^L_{\max} + ||G^{1/2}||_{\infty}^2W )) \tau^{\mix}(\alpha_K) \alpha_0 \nonumber
% \end{align}
% The equality follows from~\Cref{lem:non-randomness:z_0}.
% For \( k \geq K\), let \( \tau := \tau^{\mix}(\alpha_k)\).


% For \( k\leq K_{\mix}\), let \( \tau : = k\). Then, we have
% \begin{align}
%       \mathbb{E}[ \xi_k (z_k,Q_k)] \leq   \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}   k \alpha_{0}\leq  \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}   K_{\mix} \alpha_{0}  \nonumber.
% \end{align}

% The first inequality follows from the fact that \( \mathbb{E}[\xi_k (z_0,Q_0)]=0\) due to non-randomness of \(z_0\) and \( Q_0 \).

For \( k \geq K_{\mix}\), letting \(\tau=\tau^{\mix}(\alpha_k)\), we have
\begin{align}
    \mathbb{E}[\xi_k (z_k,Q_k)] &\leq  
    \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} (m\rho^{k}) + 
     \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}  \tau^{\mix}(\alpha_k) \alpha_{k-\tau^{\mix}(\alpha_k)} \nonumber \\
    &\leq \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} (m\rho^{\tau^{\mix}(\alpha_k)}) +
     \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}  \tau^{\mix}(\alpha_k) \alpha_{k-\tau^{\mix}(\alpha_k)} \nonumber \\
    &\leq  \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} \alpha_k +  \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}  \tau^{\mix}(\alpha_k) \alpha_{k-\tau^{\mix}(\alpha_k)}  \nonumber\\
    &\leq \left( \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} +  \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2} \tau^{\mix}(\alpha_k)\right)\alpha_{k-\tau^{\mix}(\alpha_k)} \nonumber,
\end{align}
where the first inequality follows from~\Cref{lem:boundedness_of_ex_xi_k_tau}. The second inequality follows from the definition of \(K_{\mix}\) in~\eqref{def:K}. The third inequality comes from the definition of mixing time in~\eqref{def:mixing_time}.
\end{proof}

\subsection{Finite time analysis under Markovian noise}\hfill\\
Now, we turn to the statement of our main results. The proof logic follows similar arguments as in the i.i.d. setting. First, we begin by deriving the convergence rate of \(z_k\). We use a generic constant \(C\) for unimportant values that change line by line.
%For simplicity, we assume \(\xi \geq \max\left\{1,\frac{8\sigma^2_{\max}(B)}{\nu^2} \right \} \). 
\begin{proposition}[Convergence rate of \(z_k\)]\label{prop:convergent_rate_z_k_markovian}
Consider the step-size in~\eqref{eq:step_size} and Markovian observation model. For any \(k\geq K_{\mix}\), we have
    \begin{align}
    \mathbb{E}[V(z_k)] \leq  \frac{C_2}{k+\xi}+\frac{C (|\mathcal{S}||\mathcal{A}|)^{5}}{(1-\gamma)^6 d_{\min}^4} \frac{\tau^{\mix}(\alpha_k)}{k+\xi}  \nonumber
    \end{align}
    where \( C_2 := \max \left\{  \frac{2(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{2}}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||^2_2 ,
    \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{9}{2}}}{(1-\gamma)^6d_{\min}^4} 
    \right\}\).
% \begin{enumerate}[{1)}]
%     \item For \( k\leq K_{\mix}\), we have,
%     \begin{align}
%         \mathbb{E}[V(z_k)] \leq  \frac{C_1}{k+\xi} + \frac{C(| \mathcal{S}| |\mathcal{A}|)^{\frac{17}{4}}}{(1-\gamma)^4 d_{\min}^2}K_{\mix} \nonumber
% \end{align} 
% where \( C_1 := \max \left(  \frac{2(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{2}}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||^2_2 ,
%     \frac{72 (|\mathcal{S}| |\mathcal{A}|)^3}{(1-\gamma)^5d_{\min}^3} 
%     \right)\).
%     \item For \(k\geq K_{\mix}\), we have
%     \begin{align}
%     \mathbb{E}[V(z_k)] \leq  \frac{C_2}{k+\xi}+\frac{C (|\mathcal{S}||\mathcal{A}|)^{\frac{17}{4}}}{(1-\gamma)^6 d_{\min}^4} \frac{\tau^{\mix}(\alpha_k)}{k+\xi}  \nonumber
%     \end{align}
%     where \( C_2 := \max \left\{  \frac{2(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{2}}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||^2_2 ,
%     \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{9}{2}}}{(1-\gamma)^6d_{\min}^4} 
%     \right\}\).
% \end{enumerate}
\end{proposition}
\begin{proof}
Following similar lines as in the proof of~\Cref{prop:lower_z_convergence_rate}, we can easily obtain the following relation
\begin{align}
        \mathbb{E}[V(z_{k+1})] &\leq \left(1- \frac{2}{k+\xi} \right) \mathbb{E}[V (z_k)] + \frac{C_1}{(k+\xi)^2} + 2\alpha_k \mathbb{E}[\xi_k (z_k,Q_k) ] \nonumber,
\end{align}
where \( C_1 := \max \left\{  \frac{2(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{2}}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||^2_2 ,
    \frac{72 (|\mathcal{S}| |\mathcal{A}|)^3}{(1-\gamma)^5d_{\min}^3} 
    \right\}\).
The main difference compared to~\eqref{eq:v_low_expand} in~\Cref{prop:lower_z_convergence_rate} is that we have the non-zero term \( \mathbb{E}[\xi_k (z_k,Q_k) ]\). Now, bounding each terms, we have
% First, we consider the case when for \( k \leq K_{\mix}\).
% {\color{blue} In all equations, please replace italic fonts into roman fonts, e.g., $min$ to $\rm min$.}

% Using bound on \(\mathbb{E}[\xi_k(z_k,Q_k)]\), which is~\Cref{lem:boundedness_of_ex_z}, and the fact that \(\alpha_k\) is decreasing sequence,  we have
% \begin{align}
%     \mathbb{E}[V(z_{k+1})] &\leq (1- \frac{2}{k+\xi}) \mathbb{E}[V (z_k)] + \frac{C_1}{(k+\xi)^2} + \alpha_0^2 \frac{256(|\mathcal{S}||\mathcal{A}|)^{\frac{9}{4}}}{(1-\gamma)^4 d_{\min}^2}  K_{\mix} . \nonumber 
% \end{align}

% Hence, applying induction, we get
% \begin{align}
%     \mathbb{E}[V(z_k)] &\leq \frac{C_1}{k+\xi} + \alpha_0^2 \frac{256(|\mathcal{S}||\mathcal{A}|)^{\frac{9}{4}}}{(1-\gamma)^4 d_{\min}^2}  K_{\mix}  \label{eq:markovian_z_1} 
% \end{align}
% Now, applying bound on \(\theta\) and \(||B||_2^2\), which are~\Cref{lem:theta_bound},  and~\Cref{lem:B_upper_bound}, we can bound the last term of~\eqref{eq:markovian_z_1} as follows:

% \begin{align}
%   \alpha_0^2 \frac{256(|\mathcal{S}||\mathcal{A}|)^{\frac{9}{4}}}{(1-\gamma)^4 d_{\min}^2}  K_{\mix} 
%     &\leq  \left(\frac{\nu}{2\sigma^2_{\max}(B)}\right)^2 \frac{256(|\mathcal{S}||\mathcal{A}|)^{\frac{9}{4}}}{(1-\gamma)^4 d_{\min}^2}  K_{\mix} \nonumber\\
%     &\leq  \nu^2 \frac{(|\mathcal{S}||\mathcal{A}|)^2}{(1-\gamma)^2d_{\min}^2} \frac{256(|\mathcal{S}||\mathcal{A}|)^{\frac{9}{4}}}{(1-\gamma)^4 d_{\min}^2} K_{\mix} \nonumber \\
%     &\leq  \frac{C(| \mathcal{S}| |\mathcal{A}|)^{\frac{17}{4}}}{(1-\gamma)^4 d_{\min}^2}K_{\mix} \nonumber.
% \end{align}



% For \(k \geq K_{\mix}\), we have
\begin{align}
          \mathbb{E}[V(z_{k+1})] &\leq \left(1- \frac{2}{k+\xi} \right) \mathbb{E}[V (z_k)] + \frac{C_1}{(k+\xi)^2} \nonumber\\
    &+ 2\frac{\theta}{k+\xi} \left( \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} +  \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2} \tau^{\mix}(\alpha_k)\right) \alpha_{k-\tau^{\mix}(\alpha_k)} \nonumber  \\
         &\leq \left(1- \frac{2}{k+\xi} \right) \mathbb{E}[V (z_k)] + \frac{C_1}{(k+\xi)^2} \nonumber\\
    &+ 2\frac{\theta}{k+\xi} \left( \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2} +  \frac{64(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2} \tau^{\mix}(\alpha_k)\right)\frac{2\theta}{k+\xi} \nonumber  \\
          &=  \left(1- \frac{2}{k+\xi} \right) \mathbb{E}[V (z_k)] +  \frac{C_2}{(k+\xi)^2} + \frac{256\theta^2 (|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^4 d_{\min}^2}\frac{\tau^{\mix}(\alpha_k)}{(k+\xi)^2} \nonumber \\
          &\leq  \left(1- \frac{2}{k+\xi} \right) \mathbb{E}[V (z_k)] +  \frac{C_2}{(k+\xi)^2} + \frac{C (|\mathcal{S}||\mathcal{A}|)^{5}}{(1-\gamma)^6 d_{\min}^4} \frac{\tau^{\mix}(\alpha_k)}{(k+\xi)^2} \nonumber,
\end{align}
where the first inequality is obtained by bounding \(\mathbb{E}[\xi_k(z_k,Q_k)]\) by~\Cref{lem:boundedness_of_ex_z}, and the second inequality is due to the fact that 
\begin{align*}
    \frac{1}{k-\tau^{\mix}(\alpha_k)+\xi}\leq \frac{2}{k+\xi}, \quad \forall{k}\geq K_{\mix}.
\end{align*} 

Applying the same logic of induction as in the proof of~\Cref{prop:lower_z_convergence_rate}, we have
\begin{align}
    \mathbb{E}[V(z_k)] \leq \frac{C_2}{k+\xi}+\frac{C (|\mathcal{S}||\mathcal{A}|)^{5}}{(1-\gamma)^6 d_{\min}^4} \frac{\tau^{\mix}(\alpha_k)}{k+\xi} . \nonumber
\end{align}

This completes the proof.
% ################### telescope proof ###########

% Rearranging the terms, we have
% \begin{align}
%     \frac{1}{k+\xi} \mathbb{E}[V (z_k)]      &\leq (1- \frac{1}{k+\xi}) \mathbb{E}[V (z_k)] - \mathbb{E}[V (z_{k+1})]+ \frac{C_l}{(k+\xi)^2} + 2\alpha_k \mathbb{E}[\xi_k (z_k) ]  \nonumber
% \end{align}

% Multiplying \(k+\xi\), we have
% \begin{align}\label{ineq:lower_z_summation}
% \mathbb{E}[V (z_k)]&\leq (k+\xi-1) \mathbb{E}[V (z_k)] -(k+\xi) \mathbb{E}[V (z_{k+1})]+ \frac{C_l}{(k+\xi)} + 2\theta \mathbb{E}[\xi_k (z_k) ]  
% \end{align}

% Summing up~\eqref{ineq:lower_z_summation} from \(k=0\) to \(K-1\), we have
% \begin{align}
%   \sum_{k=0}^{K-1} \mathbb{E}[V (z_k)]&\leq  (\xi-1) \mathbb{E}[V (z_0)] -(K-1+\xi) \mathbb{E}[V (z_{K})]+ \sum^{K-1}_{k=0}\frac{C_l}{(k+\xi)} + 2\theta \sum^{K-1}_{k=0} \mathbb{E}[\xi_k (z_k) ]  \nonumber
% \end{align}

% We now bound \(\sum^{K-1}_{k=0} \mathbb{E}[\xi_k (z_k) ] \) decomposing into 
% \(\sum^{\tau^{\mix}(\alpha_K)}_{k=0} \mathbb{E}[\xi_k (z_k) ] \)
% and \(\sum^{K-1}_{k=\tau^{\mix}(\alpha_K)+1} \mathbb{E}[\xi_k (z_k) ] \).
% First note that
% \begin{align}
%     \sum_{i=0}^k \alpha_i = \sum_{i=0}^k \frac{\theta}{k+\xi} \leq \theta \log (k+\xi) \nonumber
% \end{align}
% Using~\Cref{lem:boundedness_of_ex_z}, we have
% \begin{align}
%     \sum^{\tau^{\mix}(\alpha_K)}_{k=0} \mathbb{E}[\xi_k (z_k) ] &\leq  \sum^{\tau^{\mix}(\alpha_K)}_{k=0} 
%     M\sum_{i=0}^{k-1}  \alpha_i \nonumber \\
%     &\leq \tau^{\mix}(\alpha_K) M \sum^{\tau^{\mix}(\alpha_K)-1}_{i=0}\alpha_i \nonumber \\
%     &\leq \tau^{\mix}(\alpha_K) M \theta \log(\tau^{\mix}(\alpha_K) +\xi) \nonumber\\
%     &\leq {\color{orange} \tau^{\mix}(\alpha_K) M \theta \log(K +\xi) } \nonumber.
% \end{align}
% Proceeding on, again using~\Cref{lem:boundedness_of_ex_z}, we have
% \begin{align}
%   \sum^{K-1}_{k=\tau^{\mix}(\alpha_K)+1}  \mathbb{E}[\xi_k(z_k)] &\leq \sum^{K-1}_{k=\tau^{\mix}(\alpha_K)+1}  (2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \alpha_{k-\tau^{\mix}(\alpha_K)} \nonumber \\
%   &\leq \sum^{K-1}_{k=0}  (2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \alpha_k \nonumber \\
%   &\leq  (2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \theta \log(K+\xi) \nonumber
% \end{align}
% Hence combining the terms, we have,
% \begin{align}\label{ineq_xi_k_summation}
%   \sum^{K-1}_{k=0} \mathbb{E}[\xi_k (z_k) ]  \leq  2(2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \theta \log(K+\xi) .
% \end{align}

% Applying~\eqref{ineq_xi_k_summation} to~\eqref{ineq:lower_z_summation}, we have
% \begin{align}
%       \sum_{k=0}^{K-1}\mathbb{E}[V (z_k)]&\leq  (\xi-1) \mathbb{E}[V (z_0)] -(K-1+\xi) \mathbb{E}[V (z_{K})]+ C_l \log (K+\xi) + 4\theta (2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \theta \log(K+\xi)  \nonumber
% \end{align}
% Rearranging the terms, we have
% \begin{align}
%   (K-1+\xi) \mathbb{E}[V (z_{K})] &\leq  (\xi-1) \mathbb{E}[V (z_0)] -  \sum_{k=0}^{K-1} \mathbb{E}[V (z_k)] + C_l \log (K+\xi) + 4\theta (2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \theta \log(K+\xi) \nonumber \\
%   &\leq  (\xi-1) \mathbb{E}[V (z_0)] + 4\theta (2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \theta \log(K+\xi) \nonumber
% \end{align}
% Finally, we get
% \begin{align}
%         \mathbb{E}[V (z_{K})] &\leq \frac{(\xi-1)}{K-1+\xi} \mathbb{E}[V (z_0)] + \frac{1}{K-1+\xi}4\theta (2 \frac{48(|\mathcal{S}||\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^4 d_{\min}^2}_0 + M \tau^{\mix}(\alpha_K)) \theta \log(K+\xi) \nonumber
% \end{align}

% ##########################################

\end{proof}
From~\eqref{def:z_k}, we can derive the final iterate convergence rate for \(  \mathbb{E}[|| Q^L_k-Q^* ||_{\infty}]\).
\begin{theorem}\label{thm:markovian_lower_system_convergence_rate}
For any \(k \geq K_{\text{mix}}\), we have
\begin{align}
     \mathbb{E}[|| Q^L_k-Q^* ||_{\infty}] &\leq \frac{C^L}{\sqrt{k+\xi}} + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{4}}}{(1-\gamma)^{\frac{5}{2}} d_{\min}^{\frac{3}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber,
\end{align}
where \(C^L:=  \max \left\{ C(|\mathcal{S}||\mathcal{A}|)^{3}||Q^L_0 -Q^*||_2 ,
    \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}} 
    \right\}  \).
% \begin{enumerate}[1)]
% \item For \( k \leq K_{\textbf{mix}}\), we have
% \begin{align}
%         \mathbb{E}[|| Q^L_K-Q^* ||_{\infty}] \leq
%  \frac{C^L_1}{\sqrt{k+\xi}}  + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{19}{8}}}{(1-\gamma)^{\frac{3}{2}} d_{\min}^{\frac{1}{2}}} \sqrt{K_{\text{mix}}}\nonumber,
% \end{align}
% where \(C^L_1 := \max\left\{ 2(|\mathcal{S}||\mathcal{A}|)^3 ||Q^L_0 -Q^*||_2, \frac{12(|\mathcal{S}||\mathcal{A}|)^{\frac{7}{4}}}{(1-\gamma)^2d_{\min}} \right\}\). 
% \item For \(k \geq K_{\text{mix}}\), we have
% \begin{align}
%      \mathbb{E}[|| Q^L_k-Q^* ||_{\infty}] &\leq \frac{C^L}{\sqrt{k+\xi}} + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{19}{8}}}{(1-\gamma)^{\frac{5}{2}} d_{\min}^{\frac{3}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber,
% \end{align}
% where \(C^L:=  \max \left\{ C(|\mathcal{S}||\mathcal{A}|)^{3}||Q^L_0 -Q^*||_2 ,
%     \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}} 
%     \right\}  \).
% \end{enumerate}
\end{theorem}

\begin{proof}

Noting that \( Q^L_k-Q^* = G^{-1/2} z_{k}\) and from~\Cref{prop:convergent_rate_z_k_markovian}, we have
% \begin{align*}
%     \mathbb{E}[||Q^L_k - Q^* ||_{2}^2] &\leq \lambda_{\max}(G^{-1}) \left( \frac{1}{k+\xi} \max \left\{  \frac{2(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{2}}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||^2_2 ,
%     \frac{72 (|\mathcal{S}| |\mathcal{A}|)^3}{(1-\gamma)^5d_{\min}^3} 
%     \right\} \right.\\
%     &+ \left. \frac{C(| \mathcal{S}| |\mathcal{A}|)^{\frac{17}{4}}}{(1-\gamma)^4 d_{\min}^2}K_{\mix}\right) \\
%     % &\leq 2\sqrt{|\mathcal{S}||\mathcal{A}|} (1-\gamma)d_{\min} \left( \frac{1}{k+\xi} \max \left\{  \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{2}}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||^2_2 ,
%     % \frac{144 (|\mathcal{S}| |\mathcal{A}|)^3}{(1-\gamma)^5d_{\min}^3} 
%     % \right\} \right.\\
%     % &+ \left. \frac{2^9(| \mathcal{S}| |\mathcal{A}|)^{\frac{17}{4}}}{(1-\gamma)^6 d_{\min}^4}K_{\mix} \right) \nonumber\\
%     &\leq \frac{(C_1^L)^2}{k+\xi}  + \frac{C(| \mathcal{S}| |\mathcal{A}|)^{5}}{(1-\gamma)^3 d_{\min}}K_{\mix} \nonumber.
% \end{align*}
% The inequality follows from~\Cref{lem:inv_G_bound}. Using algebraic properties of the norm and Jensen's inequality,
% \begin{align}
%     \mathbb{E}[||Q^L_k - Q^*||_{\infty}] &\leq \mathbb{E}[||Q^L_k-Q^*||_2] \nonumber\\
%     &\leq \sqrt{\mathbb{E}[||Q^L_k-Q^*||_2^2]} \nonumber \\
%     &\leq  \frac{C_1^L}{\sqrt{k+\xi}}  + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{19}{8}}}{(1-\gamma)^{\frac{3}{2}} d_{\min}^{\frac{1}{2}}} \sqrt{K_{\mix}}\nonumber
% \end{align}
% The last inequality follows from the fact that \(\sqrt{a+b}\leq \sqrt{a}+\sqrt{b} \).

%Similarly, for \( k \geq K_{\mix}\), we can derive the following bound:
\begin{align*}
    \mathbb{E}[|| Q^L_k-Q^* ||^2_2]
    &\leq \lambda_{\max}(G^{-1}) \left(  \max \left\{  \frac{8(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{2}}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||^2_2 ,
    \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{9}{2}}}{(1-\gamma)^6d_{\min}^4} 
    \right\} \frac{1}{k+\xi} \right. \\
    &\left.+\frac{C (|\mathcal{S}||\mathcal{A}|)^{5}}{(1-\gamma)^6 d_{\min}^4} \frac{\tau^{\mix}(\alpha_k)}{k+\xi} \right) \nonumber\\
    &\leq  \frac{(C^L)^2}{k+\xi}+\frac{C (|\mathcal{S}||\mathcal{A}|)^{\frac{11}{2}}}{(1-\gamma)^5 d_{\min}^3} \frac{\tau^{\mix}(\alpha_k)}{k+\xi} , \nonumber
\end{align*}
where the second inequality follows from the upper bound on \(G^{-1}\) in ~\Cref{lem:G_upper_bound}. Using Jensen's inequality as in~\Cref{thm:lower_system_convergence_rate}, the above result leads to
\begin{align}
     \mathbb{E}[|| Q^L_k-Q^* ||_{\infty}] &\leq   \frac{
     C^L}{\sqrt{k+\xi}} + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{4}}}{(1-\gamma)^{\frac{5}{2}} d_{\min}^{\frac{3}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}}. \nonumber
\end{align}
This completes the proof.
\end{proof}

Next, we derive a convergence rate for \(\mathbb{E}[||Q^U_k - Q^L_k||_{\infty}]\). The proof is similar to those of the i.i.d. setting: we use a bound on \(\mathbb{E}[||Q^L_k-Q^*||_{\infty}] \), and then apply an induction logic. The randomness of the \(Q^U_k-Q^L_k\) mainly relies on \( Q^L_k-Q^*\). Therefore the influence of Markovian noise in \(Q^L_k-Q^*\) directly affects the difference between the upper and lower comparison systems. That is, the convergence rate of \(\mathbb{E}[||Q^U_k -Q^L_k ||]\) follows that of \( \mathbb{E}[||Q^L_k-Q^* ||_{\infty}]\), and sample complexity becomes worse due to slow progress of the upper comparison system as seen in the i.i.d. case.
\begin{theorem}\label{thm:markovian_upper_system_convergence_rate}
For any \(k\geq K_{\mix} \), the difference between the upper and lower comparison systems is bounded as follows:
\begin{equation}
    \mathbb{E}[||Q^U_{k+1}-Q^L_{k+1}||_{\infty}] \leq \frac{\gamma d_{\max}C^U}{\sqrt{k+\xi}}    + \gamma d_{\max}\frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{15}{4}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber,
\end{equation}
where $C^U:= \max \left\{ C\frac{(|\mathcal{S}||\mathcal{A}|)^{4}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||_2 ,
    \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{7}{2}}}{(1-\gamma)^{\frac{7}{2}}d_{\min}^{\frac{5}{2}}} 
    \right\}$.
% \begin{enumerate}[1)]
% \item For \( k \leq K_{\mix}\), we can bound the difference of upper and lower system as follows:
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
% \setlength{\abovedisplayshortskip}{0pt}
% \setlength{\belowdisplayshortskip}{0pt}
% \begin{equation}
%      \mathbb{E}[|| Q^U_k -Q^L_k ||_{\infty}] \leq  \frac{\gamma d_{\max} C^U_1}{\sqrt{k+\xi}} + \gamma d_{\max}\frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{5}{2}} d_{\min}^{\frac{3}{2}}} \sqrt{K_{\mix}}\nonumber,
% \end{equation}
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
% \setlength{\abovedisplayshortskip}{0pt}
% \setlength{\belowdisplayshortskip}{0pt}
% where $C^U_1:= \max\left\{ \frac{C(|\mathcal{S}||\mathcal{A}|)^4}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||_2, \frac{C(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^3d_{\min}^2} \right\}$.

% \item For \(k\geq K_{\mix} \), we can bound the difference of upper and lower system as follows:
% \begin{equation}
%     \mathbb{E}[||Q^U_{k+1}-Q^L_{k+1}||_{\infty}] \leq \frac{\gamma d_{\max}C^U}{\sqrt{k+\xi}}    + \gamma d_{\max}\frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber,
% \end{equation}
% where $C^U:= \max \left\{ C\frac{(|\mathcal{S}||\mathcal{A}|)^{4}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||_2 ,
%     \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{7}{2}}}{(1-\gamma)^{\frac{7}{2}}d_{\min}^{\frac{5}{2}}} 
%     \right\}$.
% \end{enumerate}
\end{theorem}
\begin{proof}
As in~\Cref{thm:upper_system_convergence_rate}, we take expectation on~\eqref{eq:up_lr_diff}, and use sub-multiplicativity of the norm. 
% We first consider the case when \(k\leq K_{\mix}\):
% \begin{align}
% \mathbb{E}[||Q^U_{k+1}-Q^L_{k+1}||_{\infty}] &\leq 
%     ( 1- \frac{2}{k+\xi}) \mathbb{E} [||Q^U_k- Q^L_k ||_{\infty}] + 2\frac{\theta}{k+\xi} \gamma d_{\max} \mathbb{E}[||Q^L_k-Q^*||_{\infty}] \nonumber  \\
%     &\leq     ( 1- \frac{2}{k+\xi}) \mathbb{E} [||Q^U_k- Q^L_k ||_{\infty}] \nonumber\\
%     &+ \frac{2\theta}{k+\xi}\gamma d_{\max} \left( \frac{C_1}{\sqrt{k+\xi}}+ \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{19}{8}}}{(1-\gamma)^{\frac{3}{2}} d_{\min}^{\frac{1}{2}}} \sqrt{K_{\mix}}\right)  \nonumber \\
%     &\leq     ( 1- \frac{2}{k+\xi}) \mathbb{E} [||Q^U_k- Q^L_k ||_{\infty}] \nonumber\\
%     &+ \frac{\gamma d_{\max}}{k+\xi} \left( \frac{C^U_1}{\sqrt{k+\xi}}  + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{5}{2}} d_{\min}^{\frac{3}{2}}} \sqrt{K_{\mix}}\right) \nonumber,
% \end{align}
% where \(C_1:=  \max\left\{ 4(|\mathcal{S}||\mathcal{A}|)^3 ||Q^L_0 -Q^*||_2, \frac{12\sqrt{2}(|\mathcal{S}||\mathcal{A}|)^{\frac{7}{4}}}{(1-\gamma)^2d_{\min}} \right\} \).
% The second inequality follows from upper bound on the lower system,~\Cref{thm:markovian_lower_system_convergence_rate}. The last inequality follows from upper bound of \( \theta \),~\Cref{lem:theta_bound}.

% Consequently, using induction logic, we have,
% \begin{align}
%     \mathbb{E}[|| Q^U_k -Q^L_k ||_{\infty}] \leq  \frac{\gamma d_{\max}C^U_1}{\sqrt{k+\xi}} + \gamma d_{\max}\frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \sqrt{K_{\mix}}\nonumber.
% \end{align}

%For \( k \geq K_{\mix}\), under the same logic, we have the following bound:
\begin{align}
\mathbb{E}[||Q^U_{k+1}-Q^L_{k+1}||_{\infty}] &\leq 
    ( 1- \frac{2}{k+\xi}) \mathbb{E} [||Q^U_k- Q^L_k ||_{\infty}] + 2\frac{\theta}{k+\xi} \gamma d_{\max} \mathbb{E}[||Q^L_k-Q^*||_{\infty}] \nonumber \\
    &\leq  ( 1- \frac{2}{k+\xi}) \mathbb{E} [||Q^U_k- Q^L_k ||_{\infty}] \nonumber\\
    &+ 2\frac{\theta}{k+\xi} \gamma d_{\max} \left(
     \frac{C^L}{\sqrt{k+\xi}} + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{11}{4}}}{(1-\gamma)^{\frac{5}{2}} d_{\min}^{\frac{3}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}}
    \right)\nonumber\\
    &\leq ( 1- \frac{2}{k+\xi}) \mathbb{E} [||Q^U_k- Q^L_k ||_{\infty}] \nonumber\\
    &+ 2\frac{\gamma d_{\max}}{k+\xi}  \left(
     \frac{C_2^U}{\sqrt{k+\xi}} + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{15}{4}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}}
    \right) \nonumber,
\end{align}
where \( C^L := \max \left\{ C(|\mathcal{S}||\mathcal{A}|)^{3}||Q^L_0 -Q^*||_2 ,
    \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}} 
    \right\} \).
The first inequality follows from the same logic in~\Cref{thm:upper_system_convergence_rate}. The second inequality follows the upper bound on the lower comparison system,~\Cref{thm:markovian_lower_system_convergence_rate}. The last inequality follows from upper bound on \(\theta\) in~\eqref{lem:theta_bound}. Applying the same induction logic in~\Cref{thm:upper_system_convergence_rate}, we have
\begin{align}
    \mathbb{E}[||Q^U_{k+1}-Q^L_{k+1}||_{\infty}] &\leq \frac{\gamma d_{\max}C^U}{\sqrt{k+\xi}}    + \gamma d_{\max}\frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{15}{4}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber.
\end{align}
 
 
\end{proof}

Finally, we derive the convergence rate for the original system. which follows from simple triangle inequality.
\begin{theorem}\label{thm:markovian_convergence_rate}
For \(k \geq K_{\mix}\), we have
\begin{align}
    \mathbb{E}[||Q_k-Q^*||_{\infty}] &\leq   \frac{C^*}{\sqrt{k+\xi}}   + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{15}{4}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber,
\end{align}
where \( C^*:=  \max \left\{ C\frac{(|\mathcal{S}||\mathcal{A}|)^{4}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||_2 ,
    \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{7}{2}}}{(1-\gamma)^{\frac{7}{2}}d_{\min}^{\frac{5}{2}}} 
    \right\}\).
% \begin{enumerate}[1)]
%     \item For \(k \leq K_{\text{mix}}\), we have
% \begin{align}
%   \mathbb{E}[||Q_k - Q^*||_{\infty}] &\leq   \frac{C^*_1}{\sqrt{k+\xi}} + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}}\sqrt{K_{\mix}} \nonumber,
% \end{align}
% where \( C^*_1 = \max\left\{ \frac{C(|\mathcal{S}||\mathcal{A}|)^4 ||Q^L_0 -Q^*||_2}{(1-\gamma)d_{\min}}, \frac{C(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^3d_{\min}^2} \right\}  \).
% \item For \(k \geq K_{\mix}\), we have
% \begin{align}
%     \mathbb{E}[||Q_k-Q^*||_{\infty}] &\leq   \frac{C^*}{\sqrt{k+\xi}}   + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber,
% \end{align}
% where \( C^*:=  \max \left\{ C\frac{(|\mathcal{S}||\mathcal{A}|)^{4}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||_2 ,
%     \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{7}{2}}}{(1-\gamma)^{\frac{7}{2}}d_{\min}^{\frac{5}{2}}} 
%     \right\}\).
% \end{enumerate}
\end{theorem}
\begin{proof}

% The proof is based on simple triangle inequality.
% For \(k \leq K_{\mix}\), we have
% \begin{align}
%   \mathbb{E}[||Q_k-Q^*||_{\infty}] &\leq \mathbb{E}[||Q^L_k-Q^*||_{\infty}] +\mathbb{E}[||Q_k^U-Q^L_k||_{\infty}] \nonumber\\
%   %&\leq   \frac{1}{\sqrt{k+\xi}} \max\left( 4(|\mathcal{S}||\mathcal{A}|)^3 ||Q^L_0 -Q^*||_2, \frac{12\sqrt{2}(|\mathcal{S}||\mathcal{A}|)^{\frac{7}{4}}}{(1-\gamma)^2d_{\min}} \right) + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{19}{8}}}{(1-\gamma)^{\frac{5}{2}} d_{\min}^{\frac{3}{2}}} \sqrt{K_{\mix}} \nonumber\\
%   %&+\max\left( \frac{C(|\mathcal{S}||\mathcal{A}|)^4}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||_2, \frac{C(|\mathcal{S}||\mathcal{A}|)^{3}}{(1-\gamma)^3d_{\min}^2} \right) \frac{\gamma d_{\max}}{\sqrt{k+\xi}} + \gamma d_{\max}\frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \sqrt{K_{\mix}} \nonumber\\
%   &\leq  \frac{C^*_1}{\sqrt{k+\xi}} + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}}\sqrt{K_{\mix}}\nonumber.
% \end{align}

% The first inequality follows from triangle inequality, and the fact that \( ||Q^L_k-Q_k||_{\infty} \leq ||Q^L_k-Q^U_k ||_{\infty} \). The second inequality follows from~\Cref{thm:markovian_lower_system_convergence_rate} and~\Cref{thm:markovian_upper_system_convergence_rate}.

Using triangle inequality, we can derive the upper bound when \( k \geq K_{\mix}\),
\begin{align}
   \mathbb{E}[||Q_k-Q^*||_{\infty}] &\leq \mathbb{E}[||Q^L_k-Q^*||_{\infty}] +\mathbb{E}[||Q_k^U-Q^L_k||_{\infty}] \nonumber\\
%   &\leq  
%   \max \left( C(|\mathcal{S}||\mathcal{A}|)^{3}||Q^L_0 -Q^*||_2 ,
%     \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{5}{2}}}{(1-\gamma)^{\frac{5}{2}}d_{\min}^{\frac{3}{2}}} 
%     \right)  \frac{1}{\sqrt{k+\xi}} + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{19}{8}}}{(1-\gamma)^{\frac{5}{2}} d_{\min}^{\frac{3}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber \\
%     &+ \frac{\gamma d_{\max}}{\sqrt{k+\xi}}   \max \left( C\frac{(|\mathcal{S}||\mathcal{A}|)^{4}}{(1-\gamma)d_{\min}}||Q^L_0 -Q^*||_2 ,
%     \frac{C (|\mathcal{S}| |\mathcal{A}|)^{\frac{7}{2}}}{(1-\gamma)^{\frac{7}{2}}d_{\min}^{\frac{5}{2}}} 
%     \right) + \gamma d_{\max}\frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{8}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber\\
    &\leq \frac{C^*}{\sqrt{k+\xi}}   + \frac{C(|\mathcal{S}||\mathcal{A}|)^{\frac{15}{4}}}{(1-\gamma)^{\frac{7}{2}} d_{\min}^{\frac{5}{2}}} \frac{\sqrt{\tau^{\mix}(\alpha_k)}}{\sqrt{k+\xi}} \nonumber,
   \end{align}
where the first inequality is due to triangle inequality, and the second inequality follows from combining the bound on the lower comparison system,~\Cref{thm:markovian_lower_system_convergence_rate} and the difference of the upper and lower comparison systems,~\Cref{thm:markovian_upper_system_convergence_rate}. 
\end{proof}
\begin{remark}
    Since we can bound the mixing time with logarithmic term by~\Cref{lem:mixing_time_bound}, we can achieve \( \mathcal{O} \left( \sqrt{\frac{\log k}{k}} \right)\) convergence rate under Markovian observation model. However, from~\Cref{lem:markovian_sample_complexity_tail_bound}, the above result leads to sample complexity \(  \mathcal{O}\left( \frac{(|\mathcal{S}||\mathcal{A}|)^{\frac{27}{2}} }{(1-\gamma)^{14} d_{\min}^8} \right) \). This implies that without using mixing time in the step-size,  even though we can still get \( \mathcal{O} \left( \sqrt{\frac{\log k}{k}} \right) \) rate, the sample complexity can get extremely worse compared to the case when we use mixing time inte the step-size~\Cite{li2020sample,chen2021lyapunov,qu2020finite}. 
    %However, our aim is to provide \(\mathcal{O}\left(\sqrt{\frac{\log k}{k}}\right)\) convergence rate without knowledge of mixing time.
\end{remark}

\subsection{Comparitive analysis}
\import{./markovian}{compartive_analysis.tex}



==> preliminaries/technimcal_lemmas.tex <==

\begin{lemma}\label{lem:nest_convergence_rate}~\Cite{nemirovski2009robust}
Consider the sequence \(\{a_1,\dots,a_n\}\) for \(n\in\mathbb{N}\), and \(M\in\mathbb{R}\). Then, for \(j\in [n]\), if the following holds,
\begin{align}
    a_{j+1} \leq (1 -\frac{2}{j}) a_j + \frac{M^2}{2}\frac{1}{j^2},
\end{align}
then \(a_j \leq \frac{\max(M^2,\frac{a_1}{2})}{j} \).
\end{lemma}


\begin{lemma}\label{lem:weyl's inequality}~\Cite{bhatia2007perturbation}
Let \(X\) and \(Y\) be real symmetric matrices in \(\mathbb{R}^{n\times n}\). Then, for \(i \in [n]\),
\begin{align}
    |\lambda_i (X) - \lambda_i (Y) | \leq ||X-Y||_{\text{op}},
\end{align}
where \(\lambda_i\) corresponds to \(i\)-th largest eigenvalue of the matrix.
\end{lemma}

==> singular_value.tex <==

\begin{align}
    PT_{Q^*} + T_{Q^*}^TP = - I
\end{align}

As in \Cite{lakshminarayanan2018linear} take \( U= P^{1/2} \) and \(B= U^{-1}T_{Q^*}U\). Then
\begin{align}
    B+B^T = - P^{-1} \prec 0
\end{align}

Taking \( Uz_k = Q^L_{k}-Q^* \)
\begin{align}
    U^{-1}(Q^L_{k+1}-Q^*) &= (U^{-1}+\alpha_k U^{-1}T_{Q^*})(Q^L_k-Q^*) + \alpha_k U^{-1}w_k\\
    z_{k+1} &= (I+\alpha_k U^{-1}T_{Q^*}U) z_k + \alpha_k U^{-1}w_k\\
            &:= (I+\alpha_k U^{-1}T_{Q^*}U) z_k + \alpha_k \tilde{w}_k
\end{align}

Take \( X_k = I+\alpha_k U^{-1}T_{Q^*}U \). 
\begin{align}
    \lambda_{\max} (I+ \alpha_k (B+B^T) + \alpha_k^2 B^TB) &= 1 + \alpha_k (\sigma^2_{\max} (B)\alpha_k - \lambda_{\min}(P^{-1})) \\
                                                           \leq 1 + \alpha_k (\sigma^2_{\max} (B)\alpha_0 - \lambda_{\min}(P^{-1}))
\end{align}

Take \( \alpha_k = \frac{1}{k+\xi}\) where \( \xi =\max(1,\frac{\sigma^2_{\max}(B)}{\lambda_{\min}(P^{-1})}+\epsilon) \) where \(\epsilon>0\).
We need \(\xi>1\) for induction proof for convergence rate.  
Define \( \nu_k = \frac{\tau_0 \alpha_k}{2}\)
Then,
\begin{align}
    \rho(X^T_kX_k)\leq 1- \tau_0 \alpha_k := v_k <(v_k + \nu_k)^2 =  (1-\frac{\tau_0\alpha_k}{2})^2
\end{align}
where \( \tau_0 = \lambda_{\min}(P^{-1}) - \sigma^2_{\max} (B)\alpha_0 \).

Since \( \rho (X_k) \leq ||X_k||_2 \), there exists \(M_k\) such that
\begin{align}
    X^T_k M_k X_k -  (v_k + \nu_k)^2 M_k = -  (v_k + \nu_k)^2I
\end{align}



\begin{lemma}
Let \( V= x^T M_0 x \) and \( \alpha_k = \frac{1}{k+\xi} \). Then
\begin{align}
    \mathbb{E}[V(z_{k+1})] \leq \frac{G}{\hat{k}}= \frac{G\tau_0}{4(k+\xi)}
\end{align}
where \( G= \max(\tilde{W}\lambda_{\max}(M_0)\frac{16}{\tau_0^2},||z_0||^2)\)
\end{lemma}
\begin{proof}

\begin{align}
    \mathbb{E}[V(z_{k+1})|\mathcal{F}_k] &= \mathbb{E}[(z_k)^TX_k^TM_0X_k(z_k)+ \alpha_k^2 \tilde{w}_k^T M_0 \tilde{w}_k | \mathcal{F}_k]    \\
                                        &\leq (v_k + \nu_k)^2 V(z_k)  + \lambda_{\max}(M_1)\alpha_k^2 \mathbb{E}[\tilde{w}^T_k\tilde{w}_k|\mathcal{F}_k] \\
                                        &\leq (1- \tau_0 \frac{\alpha_k}{2})^2 V (z_k) + \alpha_k^2 \lambda_{\max}(M_0) \tilde{W}\\
                                        &\leq (1- 2 \frac{\tau_0}{4(k+\xi)})V (z_k) + \frac{\tau_0^2}{16(k+\xi)^2} \frac{16}{\tau_0^2} \lambda_{\max}(M_0) \tilde{W}
\end{align}

Taking \(\frac{1}{\hat{k}}= \frac{\tau_0}{4(k+\xi)}\), by~\Cref{lem:nest_convergence_rate},
\begin{align}
    \mathbb{E}[V(z_{k+1})] \leq \frac{G}{\hat{k}}= \frac{G\tau_0}{4(k+\xi)}
\end{align}
where \( G= \max(\tilde{W}\lambda_{\max}(M_0)\frac{16}{\tau_0^2},||z_0||^2)\)
\end{proof}

\begin{theorem}
\begin{align}
\mathbb{E}[||Q^L_k-Q^*||_{\infty}] \leq \sqrt{||U||_2^2 \frac{G\tau_0}{4(k+\xi)}} := \sqrt{\frac{\Bar{G}}{k + \xi }}
\end{align}
where \( G= \max(\tilde{W}\lambda_{\max}(M_0)\frac{16}{\tau_0^2},||U^{-1} (Q^L_0 - Q^*) ||^2)\).
\end{theorem}

\begin{proof}
\begin{align}
\mathbb{E}[||Q^L_k-Q^*||^2_2] &\leq \mathbb{E}[||U (z_k-z^*)||^2_2]\\
                  &\leq ||U||_2^2 \mathbb{E}[||z_k-z^*||^2_2]\\
                  &\leq ||U||_2^2 \frac{G\tau_0}{4(k+\xi)}
\end{align}
\end{proof}
